FastUMI: A Scalable and Hardware-Independent Universal Manipulation Interface with Dataset

Real-world manipulation data involving robotic arms is crucial for developing generalist action policies, yet such data remains scarce since existing data collection methods are hindered by high costs, hardware dependencies, and complex setup requirements. In this work, we introduce FastUMI, a substantial redesign of the Universal Manipulation Interface (UMI) system that addresses these challenges by enabling rapid deployment, simplifying hardware-software integration, and delivering robust performance in real-world data acquisition. Compared with UMI, FastUMI has several advantages: 1) It adopts a decoupled hardware design and incorporates extensive mechanical modifications, removing dependencies on specialized robotic components while preserving consistent observation perspectives. 2) It also refines the algorithmic pipeline by replacing complex Visual-Inertial Odometry (VIO) implementations with an off-the-shelf tracking module, significantly reducing deployment complexity while maintaining accuracy. 3) FastUMI includes an ecosystem for data collection, verification, and integration with both established and newly developed imitation learning algorithms, accelerating policy learning advancement. Additionally, we have open-sourced a high-quality dataset of over 10,000 real-world demonstration trajectories spanning 22 everyday tasks, forming one of the most diverse UMI-like datasets to date. Experimental results confirm that FastUMI facilitates rapid deployment, reduces operational costs and labor demands, and maintains robust performance across diverse manipulation scenarios, thereby advancing scalable data-driven robotic learning.

==> saved/TODO <==
\emph{Teleoperation-driven methods} rely on human operators to directly control robots for collecting high-quality interaction data, encompassing visual inputs, motor states, and action commands.
While these methods enable precise data acquisition, they are inherently labor-intensive and costly.
Tools like the SpaceMouse\footnote{https://3dconnexion.com/us/spacemouse/} offer fine-grained precision in robot control but exhibit limitations in targeting small or intricate objects.
Moreover, inherent latency in teleoperation systems can compromise task accuracy and fluidity, particularly in dynamic or time-sensitive contexts.
\emph{Vision-based demonstration approaches} utilize video recordings of human demonstrations, sourced from either curated datasets or unstructured platforms such as YouTube.
Although these methods effectively gather visual information, they often fail to capture the detailed interaction dynamics essential for robotic policies, such as precise end-effector trajectories.
\emph{Wearable sensor-based methods} employ technologies like motion-capture suits to record detailed human motion.
%haptic gloves, or IMU-based exoskeletons 
These systems effectively capture high-dimensional human actions but necessitate complex mappings to translate human behaviors into robotic embodiments, thereby limiting their direct applicability.
\emph{Sensor-enhanced interface-based frameworks}, such as the Universal Manipulation Interface (UMI)~\cite{chi2024universal}, utilize hand-held grippers equipped with integrated cameras and sensors to directly capture manipulation trajectories and multimodal interaction data.
This approach bridges the gap between human demonstrations and robotic execution by capturing task-relevant features, such as end-effector poses, with high precision.
Furthermore, these methods demonstrate high data collection efficiency, facilitating the rapid acquisition of diverse and high-quality datasets.


% Finally, \emph{preparing for future scalability} to support multimodal datasets introduced challenges in modularity and flexibility. 
% We need to design the system to accommodate additional sensors and data types in future iterations without significant redesign, requiring a forward-thinking approach to both hardware and software components.

% \vspace{.5em}
% \noindent
% \textbf{Camera Selection and Mounting.}
% The choice of the GoPro camera was deliberate. 
% Its fisheye lens captures wide-angle images that can potentially replace the combination of first-person and third-person planar cameras traditionally used in algorithms like ACT and DP.
% Our preliminary observations suggest that fisheye images from a single camera can provide sufficient spatio-temporal information, simplifying the hardware setup by eliminating the need for multiple cameras. 
% This simplification is particularly beneficial for mobile robotic arms in real-world applications, where installing multiple cameras may be impractical as there may be occlusion when using kinesthetic teaching methods.
% We mounted the RealSense T265 camera using specially designed limiters to ensure it remains perpendicular to the GoPro camera. This design choice simplifies the installation process and guarantees precise alignment between the two cameras, facilitating accurate pose estimation without the need for complex SLAM algorithms.


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\linewidth]{fig/fig_observation.pdf}
%     \vspace{-1.5em}
%     \caption{The views captured by the GoPro cameras on the handheld device and the robot-mounted device, respectively, with the red dashed line indicating the ends of the fingertips.}
%     \label{fig:alignment}
% \end{figure}



%High-quality data collection on robotic arms interactions with objects in real-world settings is critical for developing robust and generalizable action policies in robotic manipulation~\cite{bahl2022human,chi2024universal,zhaxizhuoma2024alignbotaligningvlmpoweredcustomized}. 
%Nevertheless, the limited availability of such data remains a substantial barrier to progress in this domain.
%Current data collection methodologies can be broadly classified into four representative categories: teleoperation-based approaches~\cite{zhu2023viola,ral_fan_2023,ram_zhang_2024}, vision-based demonstration techniques~\cite{bahl2022humantorobotimitationwild,levine2016learninghandeyecoordinationrobotic}, wearable sensor-based methods~\cite{}, and sensor-enhanced interface-based systems~\cite{cabi2020scalingdatadrivenroboticsreward, wang2023mimicplaylonghorizonimitationlearning,zhang2018deepimitationlearningcomplex}.

% \emph{Teleoperation-driven methods} rely on human operators to directly control robots for collecting high-quality interaction data, encompassing visual inputs, motor states, and action commands.
% While these methods enable precise data acquisition, they are inherently labor-intensive and costly.
% Tools like the SpaceMouse\footnote{https://3dconnexion.com/us/spacemouse/} offer fine-grained precision in robot control but exhibit limitations in targeting small or intricate objects.
% Moreover, inherent latency in teleoperation systems can compromise task accuracy and fluidity, particularly in dynamic or time-sensitive contexts.
% \emph{Vision-based demonstration approaches} utilize video recordings of human demonstrations, sourced from either curated datasets or unstructured platforms such as YouTube.
% Although these methods effectively gather visual information, they often fail to capture the detailed interaction dynamics essential for robotic policies, such as precise end-effector trajectories.
% \emph{Wearable sensor-based methods} employ technologies like motion-capture suits to record detailed human motion.
% %haptic gloves, or IMU-based exoskeletons 
% These systems effectively capture high-dimensional human actions but necessitate complex mappings to translate human behaviors into robotic embodiments, thereby limiting their direct applicability.
% \emph{Sensor-enhanced interface-based frameworks}, such as the Universal Manipulation Interface (UMI)~\cite{chi2024universal}, utilize hand-held grippers equipped with integrated cameras and sensors to directly capture manipulation trajectories and multimodal interaction data.
% This approach bridges the gap between human demonstrations and robotic execution by capturing task-relevant features, such as end-effector poses, with high precision.
% Furthermore, these methods demonstrate high data collection efficiency, facilitating the rapid acquisition of diverse and high-quality datasets.

% The UMI system addresses challenges in human demonstration data collection and supports action policy learning across various scenarios, but its current version still has two challenges: \emph{strong coupling with specific robotic hardware and issues stemming from the use of GoPro-based visual localization with open-source SLAM\footnote{ORB-SLAM3~\cite{campos2021orb} is used here.} in the system.}
% First, the system's strict hardware requirements—such as the necessity of using the Weiss WSG-50 gripper\footnote{https://weiss-robotics.com/servo-electric/wsg-series/}—impose limitations.
% Users must procure these specific components to directly implement UMI, increasing costs and limiting adoption among those with different robotic configurations.
% Adapting UMI to other hardware requires redesigning grippers, recalibrating cameras, performing SLAM calibration, and modifying code parameters, which are labor-intensive tasks hindering plug-and-play functionality. 
% Furthermore, these modifications often lack generalizability, complicating application across different laboratories and equipment.
% Second, using the GoPro camera combined with open-source SLAM for visual localization introduces a series of issues.
% The most critical problem is the inability of ORB-SLAM3 to handle temporary visual occlusion, compounded by the fact that the GoPro hardware lacks a high-precision IMU.
% This limitation makes UMI incapable of completing tasks that involve brief visual loss, such as manipulating hinged objects, which we identified as a  significant failure case.
% As a result, the usability of the collected data for training is severely impacted; without accurate end-effector coordinates due to SLAM failures, the data becomes unusable for learning, further reducing collection efficiency.
% In addition to this fundamental issue, the system's reliance on SLAM adds considerable complexity.
% SLAM performance is highly sensitive to the parameter settings of the handheld device, and its deployment and debugging processes are time-consuming and challenging.
% Moreover, the system requires global coordinate calibration with multiple conversion steps, which significantly reduces user-friendliness.


% To achieve these objectives, we adopt a decoupled design philosophy.
% We attach finger extensions identical to those on the handheld device to the robot's gripper, aligning the robotic system with the UMI handheld apparatus. 
% By equipping existing robot grippers with these attachments, we ensure consistent observation perspectives, allowing models trained on handheld-collected data to be directly applied to real robots. 
% % We design finger attachments in multiple sizes to accommodate various gripper dimensions and shapes, utilizing a hollow design for flexible fitting. 
% % This approach enhances system versatility across multiple gripper types. 
% While retaining the GoPro camera as in the UMI system, our mechanical design ensures precise alignment the camera's viewpoint with the fingertips across different hardware configurations.
% We also refine the handheld device's mechanical structure to improve stability and durability.
% Unlike UMI, which relies on a SLAM algorithm, we directly use the RealSense T265 camera\footnote{https://dev.intelrealsense.com/docs/depth-and-tracking-cameras-alignment} which, equipped with a high-precision IMU, is capable of handling temporary visual loss, addressing a critical limitation of SLAM-based approaches.
% Additionally, this approach eliminates the need for complex SLAM deployment and calibration, thereby simplifying data processing.
% Our method requires no repetitive extrinsic calibration, simplifying both software and hardware integration.
% To ensure that Fast-UMI almost meets UMI system performance while reducing costs and simplifying deployment, we rigorously test its observation consistency and data collection process. 
% Consequently, we develop an integrated solution that combines the handheld device with robot-mounted equipment, providing an efficient and user-friendly tool for robotic learning data collection.


% We have collected over 10,000 demonstration trajectories across 20 everyday tasks to comprehensively evaluate our system. This evaluation focused on key aspects such as data collection efficiency, SLAM accuracy, data quality, and the performance of baseline algorithms like ACT on our platform. 
% Through extensive experimentation, we also derive insights into effective data collection methodologies and systematically highlighted the limitations of existing systems.


% \item \emph{Laying the groundwork for enhanced scalability to support multimodal datasets}: The redesigned interface is prepared to accommodate various data types and sensors, such as tactile sensors, allowing for the potential collection of multimodal datasets to support more complex robotic learning tasks in future iterations. 



% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=1.0\linewidth]{fig/fig_error.pdf}
%     \vspace{-1.5em}
%     \caption{Evaluation of the \emph{RealSense T265} trajectory accuracy compared to motion capture (MoCap) ground truth data. 
%     (a) Spatial trajectories along three axes: T265 measurements (red lines) and MoCap ground truth (green lines). 
%     (b) Positional errors of the T265 sensor relative to MoCap along the three axes.}
%     \label{fig:eval_t265}
% \end{figure*}

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=1\linewidth]{fig/fig_demo.pdf}
%     \vspace{-1.5em}
%     \caption{The task involves robotic manipulation to grasp a cup and place it into a sink. 
%     The first three images depict a human operator utilizing the FastUMI interface-mediated manipulation device to collect demonstration data. 
%     The subsequent two images show the robot executing an inferred action policy, trained on the collected data using the ACT algorithm.}
%     \label{fig:device1}
% \end{figure*}



%%%%%%%%%%%%%%%%%%%%

% 抽帧问题 
% 在多传感器数据融合的应用中，不同传感器的采样频率和数据模式差异常常导致数据对齐的复杂性。为了确保高质量的数据集，必须有效地解决数据同步对齐问题。为此我们提出了一种基于抽帧的对齐方法，以实现不同模态数据在统一时间戳上的精准对齐。在我们的实验设置中，T265相机以200Hz的高频率输出位姿信息，而Gopro相机则以60Hz的较低频率输出图像数据，底层通过ROS(Robot Operation System)来进行数据传输。直接融合这两种数据源会引发以下挑战：
% 1、时间同步：不同传感器的时钟可能存在偏差，导致时间戳对齐的误差增加。
% 2、并发实时处理：多种高频率的数据采集要求系统具备高效的并行数据处理能力，以避免数据积压或丢失。
% 3、频率不匹配：高频率的数据流与低频率的数据流之间存在显著差异，直接对齐可能导致数据冗余或丢失。

% 针对上述挑战，我们分别做出以下解决方法：
% 1、采用统一的ROS时钟实现不同传感器数据在时间尺度上的一致性。每一种类型的数据使用ROS的话题通信机制实现获取，同时使用了ROS的时间戳进行标注，将不同传感器的时钟统一到ROS时钟下，便于后续多模态数据基于时间匹配的对齐操作。
% 2、设计多线程数据处理架构，实现多模态数据的并行收集，并使用buffer queue对数据进行及时保存和更新。具体而言，采用独立的线程分别处理视频数据和轨迹数据的接收与写入操作，确保每种模态的数据对应同一数据收集阶段。使用deque作为缓冲区，及时保存收集的数据，避免ROS话题数据的不断更新造成收集数据丢失，并在新一轮数据收集开始前对缓冲区进行清空。缓冲区与多线程机制的结合，确保即使在高负载情况下，数据也不会因为处理延迟而丢失，保证了系统在高频率数据采集时的稳定性和可靠性。
% 3、将两种高频数据抽帧至20Hz。一方面20Hz的频率与常见的真机数据集一致。另一方面，由于这种抽帧的方式理论上可以实现位姿信息与图像数据在时间上的完全对齐，我们选取了200Hz与60Hz的最大公约数，最大概率上实现最小的对齐误差。值得一提的是，这种采取抽帧实现多种不同模态数据对齐的方法，理论最大误差为最高频数据周期的一半(在我们的setting中，即1/400秒)。具体来说，对于收集一条9秒长的轨迹（20Hz，180帧），按照传感器的输出频率，我们会得到540帧（60Hz）的图像数据和1800帧（200Hz）的位姿信息,每一帧图像和位姿都带有统一的ROS的时钟标签。我们以低频数据为基准，即从540帧图像数据中每隔3帧抽取180帧，对于每一帧的图像数据，通过遍历所有位姿信息的时钟标签，将与该帧图像在时间上最靠近的位姿进行匹配，从而实现两类数据的时间对齐。在对我们收集数据的评估中，我们测得通过这种方式获得的位姿和图像队在时间上的平均误差小于1ms，而最大误差为2.5ms，这与我们的理论最大误差一致。总的来说，我们通过对多模态数据中的最低频数据进行均匀抽帧，以低频数据为基准，通过时钟标签的比对来为其匹配高频数据，以此实现不同频数据间的匹配，避免数据的冗余或丢失。

% 我们使用ROS(Robot Operation System)来读取两种模态的数据，通过统一的ros时钟来实现数据对齐。
% 把buffer怎么构建的稍微写一下
% 我们首先为位姿信息和图像信息设置两个空的buffer列表，用于储存来自ros topic的信息。为了抽帧到我们数据集的频率，我们需要在buffer列表中存储的数据量为传感器频率除以收集数据频率再乘以数据集中单条轨迹的帧数（例如长度为180帧的轨迹，对于T265：200/20x180=1800,对于Gopro：60/20x180=540）。我们具体的时间对齐的策略如下：以低频传感器为基准，按照抽帧频率（60/20=3）从buffer列表中抽出我们的轨迹帧数长度的数据（从Gopro的buffer列表中每三帧抽取一帧，最后得到180帧），然后从高频传感器的buffer列表中分别匹配与这180帧低频数据在时间上最接近的高频数据，最终得到180帧在时间上对齐的高频数据。在数据的连续收集中，每次buffer列表都会被清空，在新的收集轮次被触发后重新开始记录。





---



% 低置信度过滤
% T265 在生成轨迹时包含了一个置信度（Confidence）标签，用于表示 T265会 对其姿态估计结果的信心程度。置信度可以通过data.tracker_confidence节点访问，输出为：0，Failed；1 Low；2 Medium；3 High。

% 影响T265置信度的因素主要有三个：1.加速度，当加速度过大时， T265会因为丢失视野而导致置信度降低。2.光线。当光线较暗时会导致置信度下降。3. 15米内景物不够。景物的缺少会导致t265无法得到足够的特征点，从而导致置信度下降。

% 收集数据时，我们首先需要测试当前场景的条件是否合格。我们需要在场景中采集一条任务轨迹，判断T265输出的任务轨迹的点的 High 置信度是否超过95%。

% 在确认场景后开始采集数据。采集过程中将同时记录轨迹点和置信度。当置信度不是High时，当前轨迹点将被舍弃，并通过前后帧插值来补充当前点。

% 平滑度
% 通过分析关节位置和姿态的变化情况来评估轨迹数据的平滑性。
% 利用位置数据的离散差分除以时间步长 Δt，计算每一时间步的速度向量；对速度数据再次进行离散差分除以时间步长，得到每一时间步的加速度向量。
% 将四元数 \(q_i\) 和 \(q_{i+1}\) 转换为旋转矩阵，并计算相对旋转 \(\Delta R = R_i^{-1} \cdot R_{i+1}\)后提取相对旋转的角度幅度 \(\theta_i\) 作为旋转角度变化。
% 设定速度、加速度和旋转角度的阈值，找到大于阈值的异常点作为轨迹中的不平滑点。




% Interchangeable fingertip modules establish standardized physical interaction points, supporting compatibility with various robotic and handheld grippers. 
% % To accommodate different robotic grippers, we have designed customized fingertip attachments for each type, as shown in \textcolor{red}{Fig.~\ref{}}.
% To accommodate a wide range of robotic grippers, we have designed five customized fingertip attachments based on commonly used grippers in open-source datasets such as Open X-Embodiment~\cite{open_x_embodiment_rt_x_2023}, covering over 90\% of the grippers in these datasets.
% Since fisheye lenses can introduce edge distortion, we improved marker detection algorithm, and applied linear interpolation for intermittent detection failures. 






% \subsection{Data Preparation for Training}

% \vspace{0.5em}
% \noindent\textbf{Data Type Overview}:
% We provide two main categories of trajectory data to accommodate various imitation learning algorithms: (1) \emph{TCP trajectories} (both absolute and relative) and (2) \emph{joint-angle trajectories}. 
% In particular, absolute TCP trajectories are commonly used by DP, whereas ACT rely on absolute joint-angle trajectories. 
% Below, we briefly introduce how to get these three data formats.

% 1 数据类型概述

% 为适配大部分模仿学习算法，我们提供两大类轨迹数据：
% TCP 轨迹（包含绝对坐标系下的 TCP 轨迹与相对坐标系下的 TCP 轨迹）
% 关节角度轨迹（Joint Trajectory）
% 简要说明这三种数据格式的区别与用途：
% 绝对 TCP 轨迹
% 相对 TCP 轨迹
% 绝对关节角度轨迹

% 为了适配大部分的模仿学习算法，我们处理了原始数据并获得了两大类轨迹数据：分别位TCP轨迹数据和关节角度轨迹数据，其中TCP轨迹数据包括绝对坐标系下的TCP轨迹与相对上一帧坐标系下的TCP轨迹。绝对TCP轨迹通常用于diffusion policy等模仿学习算法，而umi中引入的方法使用相对TCP轨迹数据训练diffusion policy模型。更传统一些的，ACT等模仿学习方法则是使用绝对关节角度轨迹进行训练。

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{0.5em}
% \noindent\textbf{Raw Input Data and Assumptions:}
% Our primary raw inputs are pose estimates from the RealSense T265 camera, denoted by \( \text{pos}_i \) (position) and \( \mathbf{r}_i \) (orientation). 
% We also require the robot's URDF and the known offset between the T265 camera and the hand-held gripper center. 
% We assume the hand-held device's motion directly mirrors that of the real robot end-effector. 
% Under these assumptions, we can derive (1) absolute TCP trajectories, (2) relative TCP trajectories, and (3) absolute joint-angle trajectories.

% 2 原始输入数据与偏置信息

% 原始数据来自 RealSense T265 相机的位姿 (Pose) 信息
% 假设已知机械臂结构参数与相机至夹爪中心的偏置 (offset)，可利用这些信息转换得到三种轨迹
% 说明如何利用相机 Pose、偏置量与机械臂结构结合，为后续的坐标转换与 IK 解算做准备

% 我们的手持设备可以获取图像信息以及对应的轨迹信息，而轨迹信息的原始数据就是来自 Realsense T265 的相机位姿信息，我们称pos_i和r_i为相机的位置与旋转数据。为了获取我们所希望的轨迹数据，也即绝对TCP轨迹，相对TCP轨迹和绝对关节角度轨迹，我们首先需要假设手持设备的夹爪末端与真机设备的夹爪具有同样的动作。假设我们已知了手持设备相机至夹爪中心的偏置，还知道了机械臂在其base坐标系下的位姿，那我们就可以将原始的相机位姿信息先转化为手持设备的位姿轨迹，然后再转化为我们需要的轨迹数据。

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{0.5em}
% \noindent\textbf{Absolute TCP Trajectory Computation:}
% To obtain absolute TCP trajectories, we map each camera pose into the robot's base coordinate system by applying the known offsets and the robot's initial base pose. 
% Let \( \text{pos}_\text{base} \) and \( \mathbf{r}_\text{base} \) denote the base frame's initial position and rotation, respectively.
% Let \(\text{Off}_x\) and \(\text{Off}_z\) be the offsets between the T265 T265 camera center and the hand-held gripper center along the \( x \)- and \( z \)-axes in the camera coordinate frame. 
% For each frame \(i\), we denote the camera's position and orientation by \( \text{pos}_i \) and \( \mathbf{r}_i \). 
% We compute the absolute TCP pose \( (\text{pos}, \mathbf{r}) \) in the base frame as follows:
% \begin{align}
% \text{offset}_1 &= 
% \begin{pmatrix}
% -\,\text{Off}_x \\[4pt]
% 0 \\[4pt]
% \text{Off}_z
% \end{pmatrix}, 
% \quad
% \text{pos}_\text{T265} \;=\; \text{pos}_\text{base} \;+\; \text{pos}_i \;+\; \text{offset}_1, \\[6pt]
% \mathbf{r}_\text{T265} &= \mathbf{r}_i \;\cdot\; \mathbf{r}_\text{base}, \\[6pt]
% \text{offset}_2 &= 
% \begin{pmatrix}
% -\,\text{Off}_z \\[4pt]
% 0 \\[4pt]
% \text{Off}_x
% \end{pmatrix}, 
% \quad
% \text{pos} \;=\; \text{pos}_\text{T265} \;+\; \mathbf{r}_\text{T265} \;\cdot\; \text{offset}_2, \\[6pt]
% \mathbf{r} &= \mathbf{r}_\text{T265}.
% \end{align}
% This yields the absolute end-effector pose \((\text{pos}, \mathbf{r})\) in the base frame, which is frequently used in downstream imitation learning pipelines.

% 3 绝对 TCP 轨迹计算

% 介绍从 T265 Pose 到世界坐标系下的 TCP 位姿变换流程
% 给出具体的坐标变换与偏置计算公式
% 说明世界坐标系、T265 位姿与 TCP 位姿的对应关系，强调旋转矩阵与位置向量的处理方式

% 接下来我们介绍如何将获取的原始数据（也就是相机的位姿轨迹）转化为绝对TCP轨迹。如图所示，我们分别称Off_x与Off_z为Realsense T265相机中心到手持设备夹爪中心在x方向（沿着夹爪的方向）与ｚ方向（竖直向上的方向）的偏置距离，同时我们分别称pos_base与r_base为机械臂的初始位置关于base坐标系下的位置与旋转。
% 我们假设手持设备的夹爪与机械臂的夹爪有着同样的行为，而在任何坐标系下，相机的位姿与TCP的位姿仅相差了一个偏置，因此轨迹计算过程中，可以先计算相机在世界坐标系下的轨迹，然后通过偏置将轨迹点映射为夹爪的位姿。这样我们就获得了绝对TCP轨迹数据，也就是在base坐标系下的TCP数据。
% 具体的计算流程如下：其中pos_T265与r_T265分别表示T265在世界坐标系下的位置与旋转矩阵，pos与r则表示绝对TCP轨迹。
% \begin{align}
% \text{offset}_1 &= \begin{pmatrix} -Off_x \\ 0 \\ Off_z \end{pmatrix} \\
% \text{pos}_\text{T265} &= \text{pos}_\text{base} + \text{pos}_i + \text{offset}_1 \\
% \text{r}_\text{T265} &= \text{r}_i \cdot \text{r}_\text{base} \\
% \text{offset}_2 &= \begin{pmatrix} -Off_z \\ 0 \\ Off_x \end{pmatrix} \\
% \text{pos} &= \text{pos}_\text{T265} + \text{r}_\text{T265} \cdot \text{offset}_2 \\
% \mathbf{r} &= \text{r}_\text{T265}
% \end{align}

% 图
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{0.5em}
% \noindent\textbf{Relative TCP Trajectory Computation}:
% Relative TCP trajectories are computed by examining consecutive frames in the absolute TCP trajectory. 
% For each pair of neighboring poses, we calculate the relative position and rotation.
% This representation removes dependence on absolute frames, improving data uniformity and enhancing base-frame generalization—particularly valuable for mobile or variable-base scenarios.

% 4 相对 TCP 轨迹计算

% 介绍在获取绝对 TCP 轨迹的基础上，如何进一步计算相对轨迹
% 给出相对轨迹的定义与计算过程，附带相应公式
% 说明相对轨迹在模仿学习算法中的作用与场景

% 在获取了绝对 TCP 轨迹之后，我们可以根据计算出两帧数据之间的相对位姿变换。假设 \( \text{pos}_i, \mathbf{r}_i \) 和 \( \text{pos}_{i+1}, \mathbf{r}_{i+1} \) 是两个相邻帧的轨迹数据。相对TCP轨迹计算公式如下：
% \begin{align}
% \text{relative\_pos}_i &= \text{pos}_{i+1} - \text{pos}_i \\
% \text{relative\_r}_i &= \mathbf{r}_i^{-1} \cdot \mathbf{r}_{i+1}
% \end{align}
% 相对轨迹在模型方法算法中去除了机械臂受到的绝对TCP位姿的限制，能让数据分布更加均匀，训练出的模型具有机械臂基座位置上的泛化性。在移动平台上会有更好的应用。



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{0.5em}
% \noindent\textbf{Absolute Joint Trajectory Computation:}
% Many imitation learning methods require joint-angle data. 
% To obtain these angles, we solve inverse kinematics (IK) for each absolute TCP pose using the robot's URDF, typically with an iterative IK solver. 
% The solution from the previous frame is used as the initial guess to maintain continuity. 
% If the URDF extends only up to the flange, we incorporate the offset between the flange and the gripper center to obtain accurate joint solutions. 
% For instance, let \( \text{off\_f} \) be the distance from the flange to the gripper center. 
% Then, given \(\text{pos}\) and \(\mathbf{r}\) as the desired TCP pose, we compute:
% \begin{equation}
% \text{offset\_f} \;=\;
% \begin{pmatrix}
% 0 \\
% 0 \\
% \text{off\_f}
% \end{pmatrix},
% \quad
% \text{pos}_f \;=\; \text{pos} \;-\; \mathbf{r} \;\cdot\; \text{offset\_f},
% \end{equation}
% where \( \text{pos}_f \) is used in the IK solver to obtain the final joint configuration. 
% Thus, we can generate the absolute joint trajectories required by ACT and similar algorithms.


% 5 绝对关节角度计算（逆运动学 IK 解算）

% 介绍如何将绝对 TCP 位姿转换为机械臂的关节角度
% 简要说明 IK 解算方法（如基于 URDF 文件、迭代计算，初始关节角度选取等）
% 给出法兰盘至夹爪末端偏置的处理方式，以及如何保持解算结果在连续运动中的一致性

% 在机械臂数据中，数据类型一般分为TCP数据和关节位姿数据，适配不同类型的算法。因此我们使用IK解算，根据机械臂的URDF(Unified Robot Description Format)文件求解关节位姿。（如果要提ikpy的话，software也有已经到Bibtex Citation）。每次将当前关节位姿作为initial_position，通过ik的迭代计算，确保解算出来的关节位姿的连续一致性。对于末端仅延伸到法兰盘的URDF文件，通过修改夹爪末端到法兰盘的距离偏置可以实现IK解算。我们记pos与r分别为TCP位置与旋转矩阵，pos_f为法兰盘在世界坐标系下的位置，off_f为法兰盘到夹爪的距离。pos与pos_f的关系如下：
% \text{offset\_f} = \left( 0, 0, \text{off\_f} \right)^T
% \text{pos\_f} = \text{pos} - \mathbf{r} \cdot \text{offset\_f}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 6 夹爪开合信息

% 在上述三类轨迹数据之外，还需同步记录夹爪的开合或宽度信息
% 说明此信息对于模仿学习中手爪动作建模的重要性
% 简要描述与三类轨迹数据整合的方式或存储格式

% 除了计算轨迹数据，我们还需要记录每个轨迹点所对应的夹爪开合信息，作为操作器，夹爪的开合对于任务的成功率具有重要意义。我们使用的夹爪宽度计算方法实现了软硬件解耦：umi原版代码是通过将鱼眼镜头取畸变后转化为了他们特制的平动夹爪的实际距离，这套转化过程中涉及了很多这个平动夹爪的参数。为了与适配更多的夹爪实现硬件解构，我们检测图像中marker的角点信息并计算两个maker的中心像素距离，将像素距离线性映射到夹爪的控制命令中。这样就无需依赖特定的硬件参数。基于像素距离的映射方式使得系统可以方便地与不同尺寸、形状的夹爪进行兼容，降低了硬件变动带来的复杂性。

% 我们使用附在夹钳上的 ArUco 标记来检测夹钳宽度。为了对获取的夹爪宽度进行归一化，我们首先获取了两个超参数，即在夹爪宽度最大和最小时候，两个标记之间相应的像素距离，分别记为marker_max和marker_min。我们对数据的每一帧图像中的标记位置进行识别，获取标记的像素位置。如果识别到全部标记，就直接计算像素距离，如果识别到一个标记，那就计算与这个标记位置与水平对称位置的像素距离。如果任何帧未能检测到所有标记，则会插入夹持器宽度以确保数据完整。这样就可以保证每一帧都有一个对应的像素距离（marker＿distance）。然后我们基于下面的公式计算出夹爪的真实宽度：
% distances文件中的字段包含config.json图像中标记的最大和最小像素距离（marker_max和marker_min），以及机器人的实际最大夹持器宽度（gripper_max）。
% \text{gripper\_width} = \frac{\text{marker\_distance} - \text{marker\_min}}{\text{marker\_max} - \text{marker\_min}} \times \text{gripper\_max}
% 获取每一帧对应的夹爪宽度信息之后，我们图像、夹爪宽度、轨迹（TCP或者关节角度轨迹）信息合并在一起作为我们的最终数据形式。

% In addition to raw data acquisition, we perform several post-processing steps to convert raw sensor outputs into robot-centered state representations suitable for various learning algorithms. These steps include trajectory transformation, gripper aperture detection, inverse kinematics, and format preparation for different algorithmic pipelines.

% \subsubsection{Trajectory Transformation}
% The core tracking data originate from the RealSense T265, which provides the pose of the sensor rather than the tool center point (TCP). To map the T265 output to a robot's world-frame TCP pose, we introduce offset parameters along the $x$- and $z$-axes (\(\text{Off}_x\), \(\text{Off}_z\)). Let \(\mathbf{pos}_i\) and \(\mathbf{r}_i\) denote the position and rotation from the T265 sensor, while \(\mathbf{pos}_\text{base}\) and \(\mathbf{r}_\text{base}\) represent the robot's base frame in the world coordinate system. We first compute the T265 pose in the world frame, then apply the offset to obtain the TCP pose:
% \begin{align}
%    \mathbf{pos}_\text{T265} &= \mathbf{pos}_\text{base} + \mathbf{pos}_i, \\
%    \mathbf{r}_\text{T265} &= \mathbf{r}_\text{base} \times \mathbf{r}_i, \\
%    \mathbf{pos} &= \mathbf{pos}_\text{T265} + \mathbf{r}_\text{T265} \bigl[ : , 2 \bigr] \cdot (\!- \text{Off}_x) 
%    \;-\; \mathbf{r}_\text{T265} \bigl[ : , 0 \bigr] \cdot \text{Off}_z, \\
%    \mathbf{r} &= \mathbf{r}_\text{T265}.
% \end{align}
% Here, \(\mathbf{pos}\) and \(\mathbf{r}\) denote the TCP position and rotation, respectively. The offset values are stored in a configuration file, enabling flexible adaptation to different gripper geometries or sensor placements.

% 3.1 轨迹变换（%添加点公式这里。把坐标系转换搞清楚）
% 原始数据由RealSense T265轨迹组成。
% 为了将FastUMI采集到的数据映射为机械臂在世界坐标系下的TCP位姿，我们需要添加偏移量以将 T265 轨迹转换为 TCP（工具中心点）轨迹，我们称Off_x与Off_z作为T265到FastUMI夹爪中心在x方向（沿着夹爪的方向）与ｚ方向（竖直向上的方向）的偏置距离。pos_i和r_i为FastUMI所采集的源位置与旋转数据，也就是T265的真实轨迹。因此我们的轨迹变换的方法是先计算T265在世界坐标系下的轨迹，然后通过偏置将轨迹点映射为夹爪的位姿。具体的计算公式如下，其中pos_T265与r_T265分别表示T265在世界坐标系下的位置与旋转矩阵，pos_base与r_base表示机械臂的初始位置关于世界坐标系的位置与旋转，最终pos与r表示映射的TCP在世界坐标系下的位置与旋转

% \begin{align}
% \mathbf{Offset} = \left(－Off_x & 0 & Off_z \right)^T
% \text{pos\_T265} = \text{pos\_base} + \text{pos\_i} + \text{offset}
% \text{r\_T265} = \mathbf{r_i} \times \mathbf{r\_base}
% \text{pos} = \text{pos\_T265} + \text{r\_T265}[:, 2] \cdot \text{off\_x} - \text{r\_T265}[:, 0] \cdot \text{off\_z}
% \mathbf{r} = \text{r\_T265}
% \end{align}

% 在此过程中应用坐标变换将 T265 轨迹映射到 TCP 轨迹。
% offset文件中的字段包含config.jsonT265 到 TCP 转换在 x 轴和 z 轴方向的偏移。


% \subsubsection{Inverse Kinematics Computation}
% Although many tasks can be learned directly in TCP space, some algorithms (e.g., joint-based policies) require joint angles. We therefore implement a straightforward inverse kinematics (IK) procedure. Given the end-effector pose \((\mathbf{pos}, \mathbf{r})\), we adjust the reference to the robot's flange frame by subtracting the known flange-to-gripper offset \(\text{off\_f}\). By supplying each pose and an initial joint guess to a standard iterative IK solver (e.g., based on the URDF model and \texttt{ikpy}), we obtain consistent joint angles for each timestep:
% \[
%    \mathbf{pos}_f \;=\; \mathbf{pos} \;-\; \mathbf{r}\,\cdot \bigl(0,0,\text{off\_f}\bigr)^T,
% \]
% and \(\mathbf{pos}_f\) is then used to solve for the robot's joint configuration.


% 3.3 逆运动学（IK）计算（%这里得补充一下细节，怎么算得ik）
% 实现了简单的IK计算，将TCP数据转换为机械臂相应的绝对关节角度，方便ACT模型的训练。
% 要计算 IK，必须获得 TCP 到法兰的距离。文件distances中的字段config.json将此距离包含为flange_to_tcp。

% 在机械臂数据中，数据类型一般分为TCP数据和关节位姿数据，适配不同类型的算法。因此我们使用IK解算，根据机械臂的URDF(Unified Robot Description Format)文件求解关节位姿。（如果要提ikpy的话，software也有已经到Bibtex Citation）。每次将当前关节位姿作为initial_position，通过ik的迭代计算，确保解算出来的关节位姿的连续一致性。对于末端仅延伸到法兰盘的URDF文件，通过修改夹爪末端到法兰盘的距离偏置可以实现IK解算。我们记pos与r分别为TCP位置与旋转矩阵，pos_f为法兰盘在世界坐标系下的位置，off_f为法兰盘到夹爪的距离。pos与pos_f的关系如下：
% \text{offset\_f} = \left( 0, 0, \text{off\_f} \right)^T
% \text{pos\_f} = \text{pos} - \mathbf{r} \cdot \text{offset\_f}


% \subsubsection{Generating Different Data Formats}
% For adaptability across diverse learning frameworks, we provide separate pipelines to generate either absolute joint angles or TCP trajectories. Specifically:
% \begin{itemize}
%    \item \texttt{data\_processing\_to\_joint.py} computes the joint-space representation via the IK procedure.
%    \item \texttt{data\_processing\_to\_tcp.py} produces the TCP-space representation alongside gripper aperture data.
% \end{itemize}
% To ensure broader compatibility (e.g., with Diffusion Policy), we offer \texttt{data\_processing\_tcp\_to\_dp.py} for converting HDF5 TCP data into the Zarr format. Zarr is comparable to HDF5 yet provides enhanced flexibility in chunking, compression, and parallel I/O, facilitating efficient data handling in large-scale experiments.

% 这里只需要写我们有三类数据格式，aboslute joint trajectory，aboslute tcp pose, relative tcp pose 

% 3.4 不同类型的数据处理
% 为了适应不同类型的算法，脚本data_processing_to_joint.py和data_processing_to_tcp.py分别提供了生成机械臂绝对关节角度和TCP数据的方法。具体来说就是首先通过3.1节的轨迹变换方法，将原始数据转换为机械臂绝对TCP数据，并使用3，2节的夹持器宽度检测方法获取夹爪的宽度，最后如果有需要，则使用逆运动学算法计算出机械臂的绝对关节角度。
% 为了确保与其他 UMI-Like 数据集的兼容性并方便适应Diffusion Policydata_processing_tcp_to_dp.py ，我们提供了将 TCP 数据从 HDF5 格式转换为Zarr的脚本，作为训练数据集的容器。Zarr 与 HDF5 类似，但在存储后端、分块、压缩和并行访问方面提供了更好的灵活性。


% \subsubsection{Gripper Aperture Detection}
% We attach ArUco markers to the gripper tips to measure the gripper's opening width. Two hyper-parameters, \(\text{marker\_max}\) and \(\text{marker\_min}\), capture the pixel distance between markers when the gripper is fully open or fully closed. Let \(\text{marker\_distance}\) be the instantaneous pixel distance between markers in a given frame. If only one marker is detected, the distance is computed by reflecting the single marker's position horizontally; if none are detected, a gap is interpolated to maintain consistency. The actual gripper width is then derived as:
% \[
%    \text{gripper\_width} \;=\; \frac{\text{marker\_distance} - \text{marker\_min}}{\text{marker\_max} - \text{marker\_min}} \;\times\; \text{gripper\_max}.
% \]
% Here, \(\text{gripper\_max}\) is the gripper's physical maximum opening, also stored in a configuration file.



% 3.2 夹持器宽度检测

% 软硬件解耦：umi原版代码是通过将鱼眼镜头取畸变后转化为了他们特制的平动夹爪的实际距离，这套转化过程中涉及了很多这个平动夹爪的参数。为了与适配更多的夹爪实现硬件解构，我们检测图像中marker的角点信息并计算两个maker的中心像素距离，将像素距离线性映射到夹爪的控制命令中。这样就无需依赖特定的硬件参数。基于像素距离的映射方式使得系统可以方便地与不同尺寸、形状的夹爪进行兼容，降低了硬件变动带来的复杂性。

% 我们使用附在夹钳上的 ArUco 标记来检测夹钳宽度。为了对获取的夹爪宽度进行归一化，我们首先获取了两个超参数，即在夹爪宽度最大和最小时候，两个标记之间相应的像素距离，分别记为marker_max和marker_min。我们对数据的每一帧图像中的标记位置进行识别，获取标记的像素位置。如果识别到全部标记，就直接计算像素距离，如果识别到一个标记，那就计算与这个标记位置与水平对称位置的像素距离。如果任何帧未能检测到所有标记，则会插入夹持器宽度以确保数据完整。这样就可以保证每一帧都有一个对应的像素距离（marker＿distance）。然后我们基于下面的公式计算出夹爪的真实宽度：
% distances文件中的字段包含config.json图像中标记的最大和最小像素距离（marker_max和marker_min），以及机器人的实际最大夹持器宽度（gripper_max）。
% \text{gripper\_width} = \frac{\text{marker\_distance} - \text{marker\_min}}{\text{marker\_max} - \text{marker\_min}} \times \text{gripper\_max}


% dp(不用写，这个相当于是baseline), dp+depth （（这个相当于是baseline的基础上加模块1））

% DP: To test the usability of data collected by FastUMI, we also deployed diffusion policy using our data. We followed the same framework as UMI's (relative pose and latency matching) and it showed good results. However, we noticed that diffusion policy performed poorly when handling tasks requiring in-depth precision. For example, it sometimes couldn't reach the target or closed grippers too early. So we decided to integrate depth information into diffusion policy to improve its performance. We used the open-source depth estimation tool 'Depth Anything V2'. Since our original images contain black margins and this seriously impacts the performance of Depth Anything V2, we made some modifications to our images. To eliminate the black margins, we cropped the images to keep only the rectangles inscribed in the ellipses. Then the images were resized to 448*448 as this is the shape required by diffusion policy dataloader. After that, we used Depth Anything V2 base model to generate depth maps for these resized images. The depth maps were then concatenated to the images as their fourth channel besides RGB. For real-time inference during diffusion policy rollout, we implemented Depth Anything V2 using TensorRT and the tested inference frequency of Depth Anything V2 could reach around 50 Hz, which satisfied our requirement. According to our experiment results, ...


% liukehui update：
% 潦草版：
% To test the usability of data collected by FastUMI, we also deployed diffusion policy using our data. We followed the same framework as UMI's (relative pose and 与我们机器人特定的latency matching) and it showed good results. However, we noticed that diffusion policy performed poorly when handling tasks requiring in-depth precision. For example, it sometimes couldn't reach the target or closed grippers too early. So we decided to integrate depth information into 我们采集的数据中 to improve the performance of diffusion policy.由于在我们当前的的采集设备中没有获得实时的深度信息，因此我们采用后处理的方式为我们每一帧的数据补充对应的深度图， using the open-source depth estimation tool 'Depth Anything V2'. Since our original images 是圆形的形状并且 contain black margins and this seriously impacts the performance of Depth Anything V2, we made some modifications to our images. 通过我们的实验发现，深度信息更多是为了帮助判断夹爪与被操作物体之间的位置。因此，To eliminate the black margins, we cropped the images to keep only the rectangles inscribed in the ellipses and resized the images to 448*448. 这既保证深度图像的生成质量，又更关注于与夹爪相关的操作区域。在训练时，我们将单通道的深度信息拓展成三通道的伪彩色图，然后使用a ViT-based CLIP visual encoder (ViT-Base Patch16, 224x224 input)对RGB图片和伪彩色深度图进行编码，然后将编码后的embbeding进行连接. For real-time inference during diffusion policy rollout, we implemented Depth Anything V2 using large pre-trained model and the tested inference frequency of Depth Anything V2 could reach 20 Hz with RTX4090 GPU, which satisfied our requirement. According to our experiment result in Table[], 使用带有depth 信息的UMI-like 类型的数据可以在不使用更多传感器和多视角摄像头的成本下，极大缓解了当前主流的policy在仅使用第一腕部视角而导致的对精准操作任务深度不敏感的问题。

% 英文版：


Since our current data collection setup does not provide real-time depth information, we employed a post-processing approach to supplement each frame with corresponding depth maps using the open-source depth estimation tool \textit{Depth Anything V2}. Because our original images are circular in shape and contain black margins, which significantly impacted the performance of Depth Anything V2, we modified the images to address this issue. Through the experiments, we found that depth information primarily aids in determining the positional relationship between the grippers and the object being manipulated. So we cropped the images to retain only the rectangular areas inscribed within the ellipses to eliminate the black marginsand and resized them to 448x448. This ensured both the quality of the generated depth maps and a focus on the operational region associated with the grippers. During training, we expanded the single-channel depth information into a three-channel pseudo-color map, then used a ViT-based CLIP visual encoder (ViT-Base Patch16, 224x224 input) to encode both the RGB images and the pseudo-color depth maps. The resulting embeddings were concatenated for further processing. For real-time inference during the diffusion policy rollout, we implemented Depth Anything V2 using the large pre-trained model. The tested inference frequency of Depth Anything V2 reached 20 Hz with an RTX 4090 GPU.  According to the experimental results shown in Table [], using UMI-like data with integrated depth information significantly alleviates the depth insensitivity issue encountered in current mainstream policies when relying solely on the first wrist viewpoint, without the need for additional sensors or multi-view cameras. This enhances the policy's effectiveness in precision-intensive tasks.




% act+joint(不用写，这个相当于是baseline), act+joint+rnn （这个相当于是baseline的基础上加模块1）。 
% act+tcp+rnn / act+tcp+rnn+realtive （这两个跟上面的，其实没啥区别）




% \subsubsection{ACT Variant 1}

% act算法改进的原因：
% 在实验的时候我发现act在推理的时候会推理出数据集中完全没有出现过的jiont组合，例如，虽然训练数据中的 TCP 姿态一直朝下，推理结果却偶尔出现 TCP 完全朝上运动的情况。我猜测这是因为act在训练时将所有action视为一个``关节数 × chunk''的矩阵进行整体记忆，也就是模型并不完全是一组一组action学习的，而是把整个矩阵一起记了下来，可能会导致模型缺乏对关节之间关系的充分理解，从而导致了推理的时候产生不合理的关节组合。
% 这也是原版act之所以需要第三方视角的原因，第三方视角能够观测到机械臂关节的整体状态，潜在中给了关节组合一个限制。
% 所以当我们只用腕部视角来推理关节位姿组时就出现了这个问题。

% 因此在算法改进中我们有两点可以提升：
% 1. 强化action之间的时序关系
% 2. 在使用腕部视角时我们更推荐让模型直接预测tcp

% GRU擅长捕捉序列中的局部和时间依赖关系，能够有效地记忆和传递序列中的关键信息。通过在Transformer解码输出后添加GRU，可以利用Transformer捕捉全局依赖关系的能力，同时利用GRU增强对序列中局部和时间依赖关系的建模。这种组合有助于生成更加连贯和合理的action序列。

% 在训练阶段，我们同时最小化两个重构误差与加权的 KL 散度。
% 具体而言，模型首先输出两种动作序列预测：直接解码得到的 $\hat{a}$ 与经 GRU 后处理的 $\hat{a}_{\mathrm{GRU}}$，分别与真实动作序列通过 $L_1$ 范数计算重构损失。随后，我们根据 VAE 框架对潜变量分布的 $\mu$ 与 $\log \sigma^2$ 计算 KL 散度，并以超参数 $\lambda$ 进行加权。最终的目标函数可表述为：
% \[
% \mathcal{L} \;=\; \|\hat{a} - a\|_1 \;+\; \|\hat{a}_{\mathrm{GRU}} - a\|_1 
% \;+\; \lambda \;\mathrm{KL}(\mu, \log \sigma^2)\,.
% \]

% \subsubsection{ACT Variant 2}
% realtive：
% 一方面realtive是为了能够通过act推理与base解耦。另一方面使用绝对坐标时，不同样本之间可能会因为初始位置或整体平移等因素导致数值分布差异较大。而转换为相对位置后，能够去除初始位置等绝对坐标的干扰，更突出轨迹本身的形状和动态变化，不仅降低了大数值带来的学习难度，还提高了模型对平移等变换的鲁棒性；同时，不同来源或场景的轨迹数据也更容易对齐分布，从而简化模型设计，并使模型更好地捕捉瞬时运动的动态特征。


% \section{Open-sourced Dataset}
% 图1（长图）: 放一张大图20个场景+3个饼图

% 在本研究中，我们引入了 FastUMI 数据集。该数据集总计 10,000 条视频+轨迹（家庭场景？），覆盖 22 个任务、X 种物体类别和 X 种操作技能。
% 数据分析看图X：
% 任务分类？多样化物体？长时间跨度？

% 我们是N个人N个FastUMI设备采集。
% 每个任务是怎么设置的:只有操作对象的物品保持不变，其他内容随即变化，包括背景等信息。

% 采集的时候Open RViz for Visualization，Add Odometry and Image topics to visualize the data from the RealSense and GoPro cameras.
% 我们制定了质量保证标准 + 实时去观察T265是否飞离。%如果飞离怎么办？补充一下细节，回环？

% 原始数据实时传输使用cable，无线传输无法满足，因为图像很高清。

% 保存本地？后续在处理根据需求用户的，比如joint或者tcp，这里的处理包括什么？这里还有细节么？细节在下面。
% 3.4 �� 不同类型的数据处理
% 为了适应不同类型的算法，脚本data_processing_to_joint.py和data_processing_to_tcp.py分别提供了生成机械臂绝对关节角度和TCP数据的方法。
% 为了确保与其他 UMI-Like 数据集的兼容性并方便适应Diffusion Policydata_processing_tcp_to_dp.py ，我们提供了将 TCP 数据从 HDF5 格式转换为Zarr的脚本，作为训练数据集的容器。Zarr 与 HDF5 类似，但在存储后端、分块、压缩和并行访问方面提供了更好的灵活性。


% 在 FastUMI 数据集中，数据格式是什么？每个 HDF5 文件对应一个情节，并封装观察数据和动作，具体数据格式是XXXX。为什么选择hdf5?为了确保与其他 UMI-Like 数据集的兼容性并方便适应Diffusion Policydata_processing_tcp_to_dp.py ，我们提供了将 TCP 数据从 HDF5 格式转换为Zarr的脚本，作为训练数据集的容器。Zarr 与 HDF5 类似，但在存储后端、分块、压缩和并行访问方面提供了更好的灵活性。
% episode_<idx>.hdf5
% ├── observations/
% │   ├── images/
% │   │   └── <camera_name_1> (Dataset)
% │   └── qpos (Dataset)
% ├── action (Dataset)
% └── attributes/
%     └── sim = False
% 具体细节在https://github.com/RealRobotSquad/FastUMI_Data
% 每个任务的描述通过文件夹显示，比如Open Container，相同的episode放在同样的文件夹中。


% \begin{table*}[h]
% \centering
% \scriptsize
% \renewcommand{\arraystretch}{1}
% \setlength{\tabcolsep}{4pt}
% \caption{Error analysis of trajectories for different tasks (values in mm).}
% \label{tab:trajectory_errors}
% \begin{tabular}{llcccccccccccc}
% \toprule
% \textbf{Sensor} & \textbf{Task} & \textbf{Statistic} & \textbf{traj1} & \textbf{traj2} & \textbf{traj3} & \textbf{traj4} & \textbf{traj5} & \textbf{traj6} & \textbf{traj7} & \textbf{traj8} & \textbf{traj9} & \textbf{traj10} \\
% \midrule
% \textbf{T265} & Pick Cup & Max Err  & 18 & 21 & 20 & 18 & 22 & 18 & 20 & 17 & 14 & 16 \\
% & & Mean Err & 11 & 10 & 12 & 11 & 11 & 12 & 11 & 10 & 7  & 10 \\
% & & Min Err  & 4  & 2  & 5  & 2  & 5  & 5  & 2  & 1  & 1  & 2  \\
% \cmidrule{2-13}
% & Open Container & Max Err  & 34 & 28 & 39 & 32 & 34 & 34 & 25 & 26 & 30 & 31 \\
% & & Mean Err: 19, 16, 18, 17, 19, 17, 17, 17, 18, 19 \\
% & & Min Err  & 3  & 5  & 3  & 7  & 9  & 8  & 2  & 5  & 7  & 3  \\
% \cmidrule{2-13}
% & rearrange Coke & Max Err  & 53 & 32 & 34 & 32 & 32 & 41 & 36 & 47 & 51 & 41 \\
% & & Mean Err & 36 & 21 & 21 & 20 & 19 & 22 & 21 & 25 & 22 & 26 \\
% & & Min Err  & 3  & 7  & 1  & 3  & 2  & 4  & 4  & 3  & 2  & 3  \\
% \midrule
% \textbf{RoboBaton Mini} & Pick Cup & Max Err  & 30 & 29 & 38 & 25 & 32 & 36 & 35 & 32 & 42 & 38 \\
% & & Mean Err & 17 & 15 & 16 & 14 & 13 & 15 & 15 & 14 & 16 & 17 \\
% & & Min Err  & 5  & 4  & 5  & 3  & 2  & 3  & 2  & 2  & 3  & 5  \\
% \cmidrule{2-13}
% & Open Container & Max Err  & 28 & 68 & 21 & 34 & 23 & 29 & 21 & 35 & 27 & 23 \\
% & & Mean Err & 10 & 11 & 10 & 11 & 11 & 12 & 11 & 12 & 12 & 12 \\
% & & Min Err  & 1  & 4  & 4  & 0  & 2  & 3  & 3  & 1  & 3  & 1  \\
% \bottomrule
% \end{tabular}
% \end{table*}



% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.95\linewidth]{fig/error1.png}
%     \caption{T265 for pick cup 轨迹3D视图}
%     \label{fig:enter-label}
% \end{figure}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.95\linewidth]{fig/error2.png}
%     \caption{T265 for pick cup 轨迹三轴视图}
%     \label{fig:enter-label}
% \end{figure}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.95\linewidth]{fig/error3.png}
%     \caption{T265 for open container 轨迹3D视图}
%     \label{fig:enter-label}
% \end{figure}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.95\linewidth]{fig/error4.png}
%     \caption{T265 for open container 轨迹三轴视图}
%     \label{fig:enter-label}
% \end{figure}



% Table.~\ref{tab:trajectory_errors}展示了t265及viobot mini误差分析结果。
%我们通过两类典型操作任务来测量和分析t265及viobot mini的误差情况，分别是pick cup这类pick and place任务和open container这类铰链遮挡任务。
%首先，我们在t265和viobot mini上安装四个反光标识点，通过NOKOV（型号）光学动作捕捉系统给出t265及viobot mini的位姿ground truth。
% 与此同时，我们通过数据收集程序计算出t265及viobot mini在初始状态坐标系下的位姿。位姿ground truth和slam计算位姿的频率分别是100Hz和20Hz。我们将位姿ground truth和slam计算位姿数据统一到ros topic中，然后根据ros时钟来统一两者的时间戳。
%两类任务我们分别记录了10条数据用于计算误差，实验中记录的轨迹如图X所示。
% 我们记录了每个任务中10条轨迹的平均误差。实验结果如表X所示。我们通过轨迹精度评估工具evo来计算两类位姿数据的误差。

%实验结果表明，在测量t265误差的任务中，pick cup的定位精度较好，平均误差为10.379mm。有遮挡的铰链任务open container精度较差，平均误差为17.668mm。我们分析，在t265运动过程中，由于过于靠近物体导致图像被遮挡，会导致定位精度下降，从而轨迹计算误差变大。但这种遮挡带来的影响不会导致定位失效，定位性能依然保持鲁棒。并且，在采集过程中，突然的加减速、抖动等动作也会导致t265的视觉图像抖动，从而导致定位精度下降。另外，任务中姿态上过多的变化会导致t265丢失一些初始视觉图片中的定位物体信息。我们还发现，在某一任务开始采集阶段，前期轨迹精度较高，后期由于累积误差会导致精度有所下降。
%在测量viobot mini误差的任务中，pick cup的定位精度较差，平均误差为15.043mm。而有遮挡的铰链任务open container精度较好，平均误差为11.220mm，两者差距更小。实验结果表明，viobot mini相比t265表现出更好的跨任务定位的稳定性，而t265则在无视觉遮挡情况下表现出更好的定位性能。

% t265定位误差evo曲线分析
% 我们选取了pick cup任务来解释在数据采集过程中t265的slam定位误差情况。通过evo工具生成如Fig.~\ref{fig:t265_evo}所示的轨迹误差图，图中曲线代表t265 slam定位相对于动作捕捉系统定位ground truth的绝对位姿误差(Absolute Pose Error, APE)。
% 曲线整体呈现两边低，中间高的特点。
% 在采集轨迹开始阶段，由于t265视野内特征点较多，且还未有明显运动时，t265的slam定位误差相对较小；
% 定位误差相对较大点，即曲线的两个尖峰处出现在夹爪pick和place cup处，此时由于t265靠近桌面，视野内出现大面积遮挡，特征点变少，因此t265定位误差变大，但仍未失效；
% 在两尖峰之间是move cup的过程，此时t265远离桌面，定位特征变多，但仍未达到初始阶段时更丰富的特征，因此误差相对初始阶段较高，而相对pick and place阶段低；
% 在轨迹即将结束时，由于采集设备回到了初始位置，视野内特征点逐渐达到初始阶段时的状态，并且由于slam的回环检测，定位误差也相对较小。




% 我们测试了act 絕對joint 和 dp 相對tcp 的成功率，12個任務的成功率。
% 该实验对比了我们系统所采集的数据用于训练最原版的act算法（绝对joint）与dp算法（relative tcp）时的模型性能。每个任务训练数据为200条，其中每50条为一组，这一组内轨迹起始位置相同，场景相同，但是被操作物品位置在一个范围内变动。每组之间轨迹起始位置不同，场景不同。训练不同模型的数据完全一样.
%测试时，操作物品所处的位置都是数据集中出现过的位置，场景布置不变，但是全部是数据集中没有出现过的场景。每个任务测试15次，计算成功率。

% Table X来看，我们采集的数据支持两种不同的算法（DP 和 ACT），在多个任务中均取得了较高的成功率，说明数据集的多样性和通用性能够满足不同算法对训练样本的需求。
% 尤其是在视线遮挡较为明显的任务中，例如Rearrange Coke和Open Container等，我们系统所采集的数据精度仍然支持模型高效的完成任务。



% 在铰链式物品的操作中我们发现，随着任务对操作深度预测精度要求的提升，方法在深度预测上的不准确性对其成功率造成了显著影响。这个问题同样暴露在所有被操作物品非常短浅的任务中，如Open Drawer，Pick Lid，Pick Pen。在Open Ricecooker 任务中，DP的操作深度预测难以完成按压动作。

% Open Suitcase任务中，
% ACT模型在操作深度推理要优于dp。但是ACT模型对任务轨迹的敏感度不如dp。
% 在Pick Bear任务中，机械臂需要完全将夹爪旋转到头朝下的位姿后再操作物品。但是这对于act在腕部视角下直接推理jiot位姿形成了挑战。测试时，我们发现act在推理的时候会推理出数据集中完全没有出现过的jiont组合，例如，虽然训练数据中的 TCP 姿态一直朝下，推理结果却出现 TCP 完全朝上运动的情况。我们推测这是因为act在训练时将所有action视为一个``关节数 × chunk''的矩阵进行整体记忆，也就是模型并不完全是一组一组action学习的，而是把整个矩阵一起记了下来，可能会导致模型缺乏对关节之间关系的充分理解，从而导致了推理的时候产生不合理的关节组合。这也是原版act之所以需要第三方视角的原因，第三方视角能够观测到机械臂关节的整体状态，潜在中给了关节组合一个限制。

% 这个问题同样暴露在Pick Pen和Sweep Trash任务中。
% 在测试 Sweep Trash 任务时，我们还发现了一个额外的问题：由于数据集中包含部分超出 xArm 机械臂工作空间的轨迹，导致基于绝对位姿预测的 act 模型常常会输出机械臂无法到达的目标位置。相比之下，采用相对位姿推理的 dp 模型在一定程度上能够缓解这一问题：一方面，相对位姿的使用可以在一定程度上与机械臂基坐标系相解耦；另一方面，模型的预测往往采用增量式的小范围移动，使机械臂在执行过程中轨迹点之间的衔接更加平稳顺畅好实现。

% Sweep Trash任务中夹爪需要抓取扫帚然后用扫帚将纸团推进dustpan中。这种复杂任务对现阶段所有模型都是种挑战。


% 对于dp，我们选择任务Pick Lid和Open Ricecooker。这是因为操作深度预测不准确的问题在这两个任务中最为突出。

% 加入深度信息后（DP + Depth），dp算法的成功率显著提升。在两个任务中分别提高了26.67%和73.33%。由此可见，结合深度信息的DP算法在提高操作任务的成功率方面表现出了极大的潜力，特别是在涉及物体精确感知和操作的复杂任务中，深度信息能够显著增强算法的感知能力和决策效果。


%简单聊一下模仿学习的发展，特别是act和dp的方法探讨，主要放在模仿学习对遇到umi这类数据集所经受的挑战。
% liukehui update
% 中文版：
% 与严重依赖人类编程和针对不同类型的任务设计特定的奖励函数不同，模仿学习是一种通过学习专家示例来来使机器人获得自主执行任务能力的方法。
% 模仿学习通常被定义为两大主要类别：行为克隆和逆向强化学习。此外，对抗式模仿学习通过逆向强化学习最大化构建的对抗奖赏函数来模仿专家学习。
% 近年来，随着机械臂操作数据集的大规模收集，模仿学习被广泛运用到了机械臂操作领域上来，并且在各种类型的操作任务中都起到了振奋人心的作用。根据所收集到的机械臂数据类型的不同，不太的模仿学习算法可以学习从真实机械臂获取的数据，从无动作标签的视频中进行学习，从与机械臂解耦的手持增强设备中进行学习。在一些涉及灵巧手的方法中，模仿学习算法还可以从人类灵巧丰富的手部示例中进行学习。在时间聚合算法中，作者等人通过模仿收集到的机械臂绝对关节位姿数据，并且对推理出的固定chunking长度的action进行时序平滑处理，实现了对双臂机器人的自主平滑控制。在YAY中，作者在ACT算法中嵌入语言模态，通过微调vison-language model，实现了与双臂机器人的语言交互。Diffusion Policy也作为一种从demonstrations学习的方法，通过条件去噪过程在机器人操作空间中生成动作，具备了Expressing multimodal action distributions，High-dimensional output space，Stable training的优点。在UMI中，作者证明了使用UMI-Like数据可以用于训练diffusion policy并得到了很好的效果。在我们的工作中，我们在ACT和Diffusion Policy上对我们的系统收集到的数据进行了验证，并且探索了不同类型的数据和增添UMI-Like 深度信息对算法的影响，这将有助于未来更多算法适配于UMI-Like类型的数据，进一步拓展UMI-Like社区的发展。
% 英文版：




% By dynamically shifting the commanded TCP based on the measured gripper width, this approach compensates for geometric changes within the gripper. In turn, fine-grained manipulation tasks become more consistent and reliable, even under significant gripper motion during operation.


% \subsection{Dynamic Error-Compensation Algorithm}
% 在测试时我们发现，在用非平动夹爪执行模型推理时，由于夹爪机械结构，夹爪闭合时实际tcp的空间位置会沿z轴向前移。这种误差的发生，会对机械臂在执行精细化操作时产生严重影响，例如抓起放置在桌面的钢笔时，会因为tcp实际空间位置比推理位置更靠近桌面而导致任务失败。因此在数据处理时，我们需要通过算法进行距离补偿。我们基于视觉估计的夹爪开合宽度，动态调整tcp的空间位置，使模型推理出更准确的可执行位姿，减小末端与目标物体的相对误差。
% 首先，通过安装于机械臂前方的相机获取抓手图像序列 $\{I_i\}_{i=1}^N$，通过marker检测夹爪宽度 $\hat{W}_i$，再将夹爪宽度线性映射到夹爪控制命令$[0,\,W_{\max}]$ 区间，以得到
% \[
% W(i) \;=\; f_{\mathrm{vision}}(I_i) \;\in\; [0,\,W_{\max}],
% \]
% $W(i)$代表传输给夹爪控制命令的值。
% 引入一个与抓手宽度 $W(i)$ 相关的补偿距离 $d(i)$，用于修正tcp在夹爪闭合时在空间中的位置。令在夹爪完全闭合（$W(i) = 0$）时补偿距离最大为 $d_{\mathrm{close}}$，而在抓手完全张开（$W(i) = W_{\max}$）时补偿距离最小为 $d_{\mathrm{open}}$。则可采用线性插值方法：
% \[
% d(i) \;=\; d_{\mathrm{close}}
% \;-\;\frac{d_{\mathrm{close}} - d_{\mathrm{open}}}{W_{\max}}
% \,W(i),
% \]
% 当抓手逐渐闭合时，机械臂的有效末端将向负 $Z$ 方向后退更多距离，以匹配真实末端相对于抓手几何中心的变化。
% 令机械臂在时刻 $i$ 的期望末端位姿由位置 $\boldsymbol{p}(i)$ 与四元数姿态 $\boldsymbol{q}(i)$ 表示。将姿态 $\boldsymbol{q}(i)$ 转换为旋转矩阵 $R\bigl(\boldsymbol{q}(i)\bigr)$ 后，令
% \[
% \boldsymbol{z}_{\mathrm{axis}}(i) \;=\; R\bigl(\boldsymbol{q}(i)\bigr)\,\hat{\boldsymbol{e}}_z,
% \]
% 其中 $\hat{\boldsymbol{e}}_z$ 表示单位 $Z$ 轴向量 $[0,\;0,\;1]^\mathsf{T}$。基于上述补偿距离 $d(i)$，修正后的末端位置可写为
% \[
% \boldsymbol{p}'(i) \;=\; \boldsymbol{p}(i) 
% \;-\; d(i)\,\boldsymbol{z}_{\mathrm{axis}}(i).
% \]
% 由此得到的 $\boldsymbol{p}'(i)$ 和原姿态 $\boldsymbol{q}(i)$ 一并作为逆运动学求解的输入：
% \[
% \boldsymbol{\theta}(i) \;=\; \mathrm{IK}\bigl(\boldsymbol{p}'(i),\;\boldsymbol{q}(i)\bigr),
% \]
% 其中 $\boldsymbol{\theta}(i)$ 表示各关节角度构成的向量。

% 这种在线补偿机制有效地减小了由于抓手几何变形（闭合或张开）导致的末端姿态偏差，使得抓取任务的过程更加精确与稳定。


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \vspace{0.5em}
% \noindent\textbf{Deployment with Unified Interface}
% % BestMan

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%算法改进实验
% 为了检测算法改进的效果，我们选择原始算法测试时问题最突出的两个任务进行测试。测试时用于act组和dp组的的训练数据和上一实验一样和训练参数也完全相同。
% 测试方式也同上

% 在act算法中，引入gru和tcp后成功率大幅提升。表明时间序列特征建模与末端工具状态信息在优化任务执行性能中具有重要意义。
%我们期望引入relative的进一步加强act模型与机械臂base的解耦能力，并去除初始位置等绝对坐标的干扰，更突出轨迹本身的形状和动态变化，提高模型对平移等变换的鲁棒性。在 Sweep Trash 任务中，我们观察到模型在复杂任务中的理解能力上升，预测的准确性有明显提高。这表明，使用相对运动数据能够更好地捕捉轨迹的动态模式，使得模型可以更加稳定地生成符合预期的运动序列。但是在Pick Bear，模型对于深度估计没有绝对位姿预测准确。模型在没有绝对位姿信息的情况下，其对物体高度的感知能力有所下降，导致抓取位置的预测准确度不及使用绝对坐标时的效果。



%此实验展示了不同摄像机设置在pick and place任务和操作铰链任务的表现上的对比分析，旨在评估摄像机视角与镜头类型对模型推理的影响。我们分别用不同摄像头采集50条数据用于训练，为摒除其他的影响因素，每组数据之间环境设置完全相同并且不变，轨迹起始点相同，但是操作物品位置在一个小范围内变动，轨迹类似。并且轨迹都是通关直接遥操机械臂获取。
% 测试时，操作物品位置是数据集中出现过的位置，环境不变，场景每组测试15次计算成功率。推理模型采用的是act-joint。
%我们发现umi-like数据中采用腕部视角的鱼眼摄像头，其性能逼近甚至匹敌结合多个视角的配置。
%鱼眼摄像头因其广角视野能够捕捉更多的环境信息，从而为模型推理提供了更加丰富的上下文信息。


% 其中一個任務做200 400 800
% 杯垫放置在5个点位，杯子放置在五个点位，每个点测三次，三次中杯把分别朝向左、中、右。模型使用的是act原版。
% 这个任务中模型不但要检测杯子和杯垫的位置，还要通过识别杯把的朝向来预测不同的轨迹。


% 说明数据量的提升切实的提升了模型的泛化能力。

% 鉸鏈任務的scaling low（没做）
% 遮擋視角的任務的slam失敗率（这个相当于放在了12个任务实验里，视线有遮挡的任务：Open Container，Rearrange Coke，Open Rice Cooker，Open Drawer，Open Roaster，Open Suitcase）
% 沒有圖像和軌跡對齊的成功率和時間戳誤差



% 適配與多種機器人
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.95\linewidth]{fig/dif3.jpg}
%     \caption{Xarm}
%     \label{fig:enter-label}
% \end{figure}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.95\linewidth]{fig/dif1.jpg}
%     \caption{flexiv}
%     \label{fig:enter-label}
% \end{figure}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.95\linewidth]{fig/dif2.jpg}
%     \caption{Z1}
%     \label{fig:enter-label}
% \end{figure}


% \vspace{.5em}
% \noindent
% \textbf{Quantitative Analysis of T265 Pose Estimation Accuracy.}
% As shown in Fig. \ref{fig:eval_t265}, subfigure (a) illustrates the spatial trajectory of the T265 sensor in red, while the MoCap system's trajectory, serving as the ground truth, is displayed in green. 
% Subfigure (b) presents the positional errors of the T265 sensor compared to the MoCap data across the X, Y, and Z axes.
% For the \emph{X-axis}, the mean positional error is $-0.0384$ $m$ with a variance of $0.00056$, indicating a slight negative bias in the T265 measurements. 
% On the \emph{Y-axis}, the mean error is $-0.0116$ $m$, with a higher variance of $0.00109$, reflecting smaller positional error but greater variability compared to the X-axis. 
% The \emph{Z-axis} demonstrates a positive mean error of $0.0212$ $m$ and the smallest variance at $0.00051$, suggesting a minor upward bias with relatively low variability.
% Overall, the T265 trajectory demonstrates an average positional error of $\mathbf{0.0237}$ $m$.
% These findings indicate that while the T265 sensor provides reasonably accurate pose estimation suitable for many robotic manipulation tasks, inherent biases and variances exist that should be accounted for in precision-critical applications.

% \vspace{.5em}
% \noindent
% \textbf{Demonstration.} We validate the FastUMI system in real-world environments by implementing an action policy inferred through the ACT algorithm trained on the collected dataset. 
% Additional demonstrations illustrating the system's performance are available on our website.
